An Advanced Framework for Ultra-Realistic Simulation and Digital Twinning for Autonomous Vehicles

Simulation is a fundamental tool in developing autonomous vehicles, enabling rigorous testing without the logistical and safety challenges associated with real-world trials. As autonomous vehicle technologies evolve and public safety demands increase, advanced, realistic simulation frameworks are critical. Current testing paradigms employ a mix of general-purpose and specialized simulators, such as CARLA and IVRESS, to achieve high-fidelity results. However, these tools often struggle with compatibility due to differing platform, hardware, and software requirements, severely hampering their combined effectiveness. This paper introduces BlueICE, an advanced framework for ultra-realistic simulation and digital twinning, to address these challenges. BlueICE's innovative architecture allows for the decoupling of computing platforms, hardware, and software dependencies while offering researchers customizable testing environments to meet diverse fidelity needs. Key features include containerization to ensure compatibility across different systems, a unified communication bridge for seamless integration of various simulation tools, and synchronized orchestration of input and output across simulators. This framework facilitates the development of sophisticated digital twins for autonomous vehicle testing and sets a new standard in simulation accuracy and flexibility. The paper further explores the application of BlueICE in two distinct case studies: the ICAT indoor testbed and the STAR campus outdoor testbed at the University of Delaware. These case studies demonstrate BlueICE's capability to create sophisticated digital twins for autonomous vehicle testing and underline its potential as a standardized testbed for future autonomous driving technologies.

==> Sections/5_DiscussionFuture.tex <==
\section{Discussion and Future Work}



==> backup.tex <==
\begin{table}[hbt!]
%   \caption{Camera Sensor Paramters}
%   \label{tab:camera}
%   \centering
%   \begin{tabular}[hbt!]{@{}r||p{0.5\linewidth} @{}} 
%     \hline
%     \textbf{Parameters} & \textbf{Definition} \\
%     \hline    
%     \tt{sensor\_tick} &  Seconds between sensor captures. \\
%     \hline
%     \tt{image\_size\_x} &  Image width in pixels. \\
%     \hline
%     \tt{image\_size\_y} &  Image height in pixels \\
%     \hline
%     \tt{gamma} &  Target gamma value of the camera. \\
%     \hline
%     \tt{fov} &  Horizontal field of view in degrees. \\
%     \hline
%     \tt{shutter\_speed} &  Camera shutter speed in seconds. \\
%     \hline
%     \tt{iso} &  The camera sensor sensitivity. \\
%     \hline
%     \tt{fstop} &  Opening of the camera lens. \\
%     \hline
%     \tt{bloom\_intensity} &  Intensity for the bloom post-process effect. \\
%     \hline
%     \tt{lens\_flare\_intensity} &  Intensity for the lens flare post-process effect. \\
%     \hline
%   \end{tabular}
% \end{table}

% \begin{table}[hbt!]
%   \caption{LiDAR Sensor Paramters}
%   \label{tab:lidar}
%   \centering
%   \begin{tabular}[hbt!]{@{}r||p{0.6\linewidth} @{}} 
%     \hline
%     \textbf{Parameters} & \textbf{Definition} \\
%     \hline    
%     \tt{channel} & Number of lasers.\\
%     \hline
%     \tt{range} &  Maximum distance to measure/raycast in meters. \\
%     \hline
%     \tt{points\_per\_second} &  Points generated by all lasers per second. \\
%     \hline
%     \tt{rotation\_frequency} &  LIDAR rotation frequency. \\
%     \hline
%     \tt{upper\_fov} &  Angle in degrees of the highest laser. \\
%     \hline
%     \tt{lower\_fov} & Angle in degrees of the lowest laser. \\
%     \hline
%     \tt{horizontal\_fov} &  Horizontal field of view in degrees. \\
%     \hline
%     \tt{atmosphere\_attenuation\_rate} &  Coeff that measures the LIDAR intensity loss per meter. \\
%     \hline
%     \tt{dropoff\_general\_rate} &  General proportion of points that are randomly dropped. \\
%     \hline
%     \tt{dropoff\_intensity\_limit} &  For the intensity-based drop-off, the threshold intensity value above which no points are dropped. \\
%     \hline
%     \tt{dropoff\_zero\_intensity} &  For the intensity-based drop-off, the probability of each point with zero intensity being dropped. \\
%     \hline
%     \tt{sensor\_tick} & Seconds between sensor captures. \\
%     \hline
%     \tt{noise\_stddev} &  Standard deviation of the noise model to disturb each point along the vector of its raycast. \\
%     \hline
%   \end{tabular}
% \end{table} 

% \begin{table}[hbt!]
%   \caption{GPS Sensor Parameters}
%   \label{tab:gps}
%   \centering
%   \begin{tabular}[hbt!]{@{}r||p{0.7\linewidth} @{}} 
%     \hline
%     \textbf{Parameters} & \textbf{Definition} \\
%     \hline    
%     \tt{sensor\_tick} &  Seconds between sensor captures. \\
%     \hline
%     \tt{noise\_alt\_bias} &  Mean parameter in the noise model for altitude. \\
%     \hline
%     \tt{noise\_alt\_stddev} &  Standard deviation parameter in the noise model for altitude.\\
%     \hline
%     \tt{noise\_lat\_bias} &  Mean parameter in the noise model for latitude.\\
%     \hline
%     \tt{noise\_lat\_stddev} & Standard deviation parameter in the noise model for latitude.\\
%     \hline
%     \tt{noise\_lon\_bias} &  Mean parameter in the noise model for longitude. \\
%     \hline
%     \tt{noise\_lon\_stddev} &  Standard deviation parameter in the noise model for longitude.\\
%     \hline
%   \end{tabular}
% \end{table}

% \begin{table}[hbt!]
%   \caption{IMU Sensor Parameters}
%   \label{tab:imu}
%   \centering
%   \begin{tabular}[hbt!]{@{}r||p{0.5\linewidth } @{}} 
%     \hline
%     \textbf{Parameters} & \textbf{Definition} \\
%     \hline    
%     \tt{sensor\_tick} &  Seconds between sensor captures. \\
%     \hline
%     \tt{image\_size\_x} &  Image width in pixels. \\
%     \hline
%     \tt{image\_size\_y} &  Image height in pixels \\
%     \hline
%     \tt{gamma} &  Target gamma value of the camera. \\
%     \hline
%     \tt{fov} &  Horizontal field of view in degrees. \\
%     \hline
%     \tt{shutter\_speed} &  Camera shutter speed in seconds. \\
%     \hline
%     \tt{iso} &  The camera sensor sensitivity. \\
%     \hline
%     \tt{fstop} &  Opening of the camera lens. \\
%     \hline
%     \tt{bloom\_intensity} &  Intensity for the bloom post-process effect. \\
%     \hline
%     \tt{lens\_flare\_intensity} &  Intensity for the lens flare post-process effect. \\
%     \hline
%   \end{tabular}
% \end{table}

% \begin{table}[hbt!]
%   \caption{DBW and Vehicle Paramters}
%   \label{tab:dbw}
%   \centering
%   \begin{tabular}[hbt!]{@{}r||p{0.6\linewidth} @{}} 
%     \hline
%     \textbf{Parameters} & \textbf{Definition} \\
%     \hline    
%     \tt{wheel\_radius} &  The radius of the wheel. \\
%     \hline
%     \tt{wheel\_width} &  The lateral width of the wheel tire. \\
%     \hline
%     \tt{wheel\_base} &  Distance between front wheel center and rear wheel center. \\
%     \hline
%     \tt{wheel\_tread} &  Distance between left wheel center and right wheel center. \\
%     \hline
%     \tt{front\_overhang} &  Distance between front wheel center and vehicle's front. \\
%     \hline
%     \tt{rear\_overhang} &  Distance between rear wheel center and vehicle's rear. \\
%     \hline
%     \tt{left\_overhang} &  Distance between left wheel center and vehicle's left. \\
%     \hline
%     \tt{right\_overhang} &  Distance between right wheel center and vehicle's right. \\
%     \hline
%     \tt{vehicle\_height} &  Vehicle's height. \\
%     \hline
%      \tt{max\_steer\_angle} &  Vehicle's maxium steering rate. \\
%     \hline
%      \tt{steer\_rate\_lim} &  Vehicle's maxium steering angle change rate.. \\
%     \hline
%     \tt{vel\_lim} &  Vehicle's maxium velocity. \\
%     \hline
%      \tt{vel\_rate\_lim} &  Vehicle's maxium acceleration. \\
%     \hline
%   \end{tabular}
% \end{table}

% As a starting point, this digital twin will be a combination of CARLA, an in-house C-V2X simulator, and SUMO. The geographical information, including the landscape, road networks, and buildings, are translated into height maps, OSM files, and meshes in the simulated world. To accurately capture the C-V2X network information, we plan to install multiple sets of Road-Side-Units (RSUs) and On-Board-Units (OBUs) along the road. The background traffic's behavior is generated according to the neutralistic driving data (NDD), which is collected in the real world through roadside units. The data is then replayed using SUMO to control background vehicles and pedestrians.

% The main goal of this digital twin is to test and validate the vehicle using high-fidelity realistic data. BlueICE is the only architecture supporting the co-simulation between general-purpose and multiple specialized simulators. With BlueICE, researchers can choose the level of detail to simulate during testing. For lower-detail testing, researchers can observe the effects of weather on camera-related algorithms. For higher-detail testing, researchers can observe how the vehicle's power train, steering, and wheels will behave in rainy weather on slippery roads. 

% For low-level detail simulation, we extract geographical information from the physical world to recreate the world in the simulated environment. First, we collected the camera and LiDAR information to recreate the building meshes. Then, we use the OSM files to recreate the road network. Next, we synchronize the weather and time of day between the physical and simulated world using cameras. For network information, we have two different methods to simulate. We can install multiple sets of RSUs and OBUs to collect the latency, range, and packet loss rate or use network simulators like NS-3\cite{RefWorks:RefID:26-rileyns-3}. The traffic information is collected using cameras and LiDARs, stored in ROSbags, and replayed in the simulated environment. The ego-vehicle information, such as width, length, height, axis, and max steering rate, is shared between the physical and the simulated environment. For low-level detail simulation, there is no need to accurately simulate details such as snow and water physics because the focus is on the proof-of-concept of the autonomous driving algorithms.

% For high-level detail simulation, the focus is on validating the autonomous vehicle before it hits the road; therefore, we need high-fidelity realistic data. By utilizing the BlueICE architecture, we can combine ground sediment simulators like IVRESS to simulate the tire track, the ground and tire compression, and the friction; we can also combine VISTA to simulate photo-realistic sensor data; we also plan to add Hardware-in-the-Loop and Vehicle-in-the-Loop simulators to better simulate our vehicle's energy consumption, communications, power train, actuation, and control modules.

To resolve this issue, current simulation research efforts are directed toward specialized simulation. For example, IVRESS\cite{RefWorks:RefID:3-ivress} focuses on simulating off-road tire tracks, and DDT\cite{RefWorks:RefID:4-dynamic} focuses on water dynamics in the surf zone. Thus, current researchers combine a mixture of general-purpose simulators, such as CARLA, and specialized simulators, such as NS-3\cite{RefWorks:RefID:26-rileyns-3} to simulate network and SUMO\cite{RefWorks:RefID:7-lopez2018microscopicsumo} to simulate traffic to test and validate autonomous driving algorithms. Unfortunately, this creates a bridging problem for researchers. Different simulators are created using different programming languages, hardware and software dependencies. For example, CARLA is designed to run on a GPU-intensive machine, but IVRESS is designed to run on High-Performance-Computers (HPCs). This incompatibility problem, be it Python version incompatibility, incompatible operating systems, or computing platform incompatibility, takes countless hours from researchers who are desperately trying to integrate different parts of their projects.

To bridge the divide between different simulators, we introduce BlueICE, the first cloud-native \textbf{Integrative Customizable} simulation \textbf{Environment}. BlueICE features an architecture that 
\begin{itemize}
    \item \textit{1) decouples the dependencies between computing platform, hardware, and software versions.}
    \item \textit{2) gives researchers the freedom to customize their testing stack and level of fidelity to suit their testing needs.}
\end{itemize}

BlueICE accomplishes this by 
\begin{itemize}
    \item \textit{1) utilizing containerization/sandboxing to decouple the dependencies between hardware and software.}
    \item \textit{2) creating a unified communication bridge between the different containers/sandboxes.}
    \item \textit{3) orchestrating the input, output, and synchronization between different simulators.}
\end{itemize}

In this paper, we will thoroughly discuss each component of the BlueICE architecture and demonstrate how we used BlueICE to create a state-of-the-art digital twin for autonomous driving testing.

To the best of our knowledge, our contributions are listed as follows:
\begin{itemize}
    \item BlueICE is the first to feature an \textbf{Integrative and Customizable} architecture for autonomous driving testing.
    \item Enable researchers to customize co-simulation to suit their research needs.
    \item Built a state-of-the-art digital twin that has the potential to become a standardized testbed for future connected and autonomous vehicles.
\end{itemize}

%However, in its integration with Autoware, it only supports up to Autoware.AI and has a limited sensor model suit. Furthermore, it is difficult to integrate it with other simulators to generate high-fidelity data.

% \TODO{CARLA. CarSim? Dengzong said in his PPT CarSim is for one-stop vehicle simulation}
% \\

% \julia{\subsubsection{Specialized simulator for vehicle simulation}}
% \TODO{put description of IVRESS and other specialized simulator here. Also describe why we need specialized simulator for vehicle simulation here. E.G. CarSim's vehicle level simulation is better than CARLA alone as they have better vehicle kinematics model, IVRESS(is it the tire simulator?) has better tire kinematics simulation than the one-stop simulator. Note: In this part, you need to say specifically that specialized simulator for vehicle simulation is also necessary.}


A simulator was defined as early as 1956 as "a computer model to represent real systems" \cite{goode1956use}. It is essential for the research and development of connected and autonomous vehicles, providing the ability to analyze the interaction between a vehicle under test (VUT) and other background vehicles when a mathematical treatment of the traffic process is infeasible or inadequate. It also offers possibilities to answer the "what if" questions for a VUT under various kinds of conditions, which can be too costly or/and too dangerous to test in the real world. They have been at the heart of the development and discussion of autonomous driving for many years \cite{kaur2021survey}. Over the past decade, studies have conducted general autonomous vehicle simulation testing in Grand Theft Auto (GTA V), TORCS GPL racing simulator, and using game engines such as Unreal Engine and Unity. In recent years, high-fidelity simulations have been developed for a specific aspect of autonomous vehicles, such as accurately simulating tire tracks in different types of terrain.

\textbf{Table \ref{tab:comparison}} compares some of the most popular simulators available to researchers. To test autonomous vehicles, the most important categories to simulate are vehicle physics, dynamic agents, sensor data, environment simulation, traffic simulation, scenario customization, and co-simulation with other platforms. In this table, a "\checkmark" denotes that the simulator supports the feature, a "x" denotes non-support, and a "\textasciitilde" indicates limited support.

Vehicle physics is a crucial component when simulating autonomous vehicles. Different vehicle models create varied vehicle physics; for instance, a truck will generate more air resistance than a sedan, and a longer axle will result in wider turns. In our comparison, almost all of the simulators support vehicle customization. The simulation of dynamic agents, traffic, and scenarios is crucial when testing AVs. Researchers need to create realistic traffic flows, including background vehicles and pedestrians, to accurately test responses. Traffic simulators primarily control these agents, while some of the compared vehicle simulators can also accomplish similar tasks but with higher computational costs.

Sensor modeling is the most crucial aspect when simulating autonomous vehicles (AVs). AVs cannot be accurately tested if the sensor models are incapable of simulating accurate and realistic sensor data. If the sensor models fail to generate realistic data, then models validated in the simulated world cannot be transferred to the real world. Most of the simulators received a "\textasciitilde" in this category, as they typically generate only medium-fidelity sensor data. The data generated by these sensor models is somewhat realistic, but distinguishable by the human eye. A "\checkmark" is given to simulators capable of producing data so realistic that it could potentially deceive the human eye.

Environment simulation also plays a significant role in testing autonomous vehicles. In the table, almost every simulator is assigned a "\textasciitilde" since, while they can simulate different weather and lighting conditions, they fall short in accurately replicating details such as tire tracks, water dynamics, and snow dynamics. These high-level details are crucial for researchers to ensure the vehicles' safety during various conditions like snow and rain. Most simulators leverage game engines for these simulations, but game engines often prioritize efficiency and typically use textures instead of physics to simulate these effects. Therefore, a "\checkmark" is assigned to specialized simulators that can accurately simulate these high-level details.



\subsection{Microsocpic(traffic) simulators}\label{LR:micro_sim}

For interactions regarding autonomous vehicles with background vehicles and traffic scenarios, microscopic traffic simulators are typically applied to generate and control the maneuvers of background traffic. Compared to macroscopic and mesoscopic simulators, microscopic traffic simulators provide simulations of individual vehicles, each with distinct characteristics and across multiple classes. Even within the same vehicle class, variations in vehicle kinematics, driver behavior, and decision-making can exist, providing diversity to background traffic and creating a more realistic traffic scenario for Connected and Autonomous Vehicles (CAVs) to navigate. In other words, CAVs interacting with background traffic controlled by microscopic simulators cannot rely on a specific, heuristic model to predict the behavior of background traffic and execute decision-making based on overly simplified models.

Various microscopic traffic simulators are available \cite{saidallah2016comparative}, including but not limited to VISSIM \cite{fellendorf2010microscopic}, AIMSUN \cite{barcelo2005dynamic}, Paramics \cite{cameron1996paramics}, and SUMO \cite{lopez2018microscopic}. Among these, VISSIM, Paramics, and AIMSUN are commercial, while SUMO is open-source. Previous works have indicated the potential for co-simulation among these platforms.

Compared to vehicle-level simulators, which will be discussed subsequently, all these microscopic traffic simulators control background vehicles using simplified, at most second-order, kinematics models (e.g. constant acceleration model, constant speed model). These simplified models enable the deployment of simulations at the network level. However, they cannot meet the requirements for evaluating vehicle dynamics, especially under extreme conditions. While designed to represent microscopic traffic patterns holistically, they effectively represent background traffic. Interactions between simulated CAVs and this background traffic can thus approximate how CAVs will behave in actual traffic, all with relatively low computational cost.


% \TODO{VISSIM, AIMSUN, Paramics, SUMO}



\subsection{Vehicle level simulators}\label{LR:vehicle_sim}
% \TODO{reorganize the content here. Ref the Webot PartC paper. This is for the one-stop vehicle simulators wrt environment and sensors and stuff}
In contrast to the microscopic traffic simulators mentioned above, vehicle-level simulators are specifically designed to more accurately simulate the kinematics and physics of an ego vehicle. In other words, they place greater emphasis on the performance and simulation of a single vehicle, potentially at the expense of the realistic control of background vehicles that microscopic traffic simulators provide. However, vehicle-level simulators excel in simulating sensor data and vehicle-level data with high fidelity, serving as an excellent platform to evaluate the performance of CAVs.

Several vehicle-level simulators exist, including LGSVL \cite{RefWorks:RefID:10-rong2020lgsvl}, CARLA \cite{RefWorks:RefID:6-dosovitskiy2017carla:}, Simulink \cite{RefWorks:RefID:18-xue2022modeling}, and Gazebo \cite{RefWorks:RefID:22-koenig2004design}. Irrespective of their providers, these simulators offer sophisticated and versatile virtual environments designed for testing and validating autonomous driving technologies, offering a wealth of features and tools that render them invaluable in the autonomous vehicle industry. They allow the recreation of complex driving scenarios and the evaluation of autonomous systems in controlled, safe environments. The extensive library of urban and suburban environments, coupled with a variety of weather conditions, facilitates comprehensive testing of autonomous vehicles under diverse conditions.

When it comes to controlling background traffic, vehicle-level simulators offer superior pedestrian motion models with detailed control to pedestrian bone movement, outperforming microscopic traffic level simulators in this regard. However, they may fall short in controlling background traffic compared to microscopic traffic simulators, given that both can generate and control background traffic. This discrepancy might be attributed to the traffic flow models such as car-following and lane change employed by microscopic traffic simulators, embedded with domain knowledge from transportation engineering. Typically, such models are not integrated into vehicle-level simulators, many of which originated from robotics simulations like Gazebo \cite{RefWorks:RefID:22-koenig2004design}.


\subsection{Multi-resolution simulator}\label{LR:co-sim}
As previously discussed, several simulators have been developed for vehicle-level simulation, offering either comprehensive solutions or specialized simulations targeting aspects like vehicle kinematics and powertrain. While vehicle-level simulation is complex and detailed, evaluating the interaction between the ego vehicle and other background vehicles is essential when assessing the interaction between ego CAV and surrounding vehicles. Controlling each background vehicle in one-stop vehicle-level simulators is computationally demanding, and occasionally, the control mechanisms for background traffic in such simulators may not align with traffic flow models. Consequently, multi-resolution co-simulation has been introduced.

NHTSA's CARMA platform, developed by the U.S. National Highway Traffic Safety Administration (NHTSA), serves to expedite the deployment of connected and automated vehicle (CAV) technologies, providing an open-source software framework as a reference for CAV systems. It amalgamates CARLA, Autoware.AI, and SUMO, utilizing Eclipse MOSAIC as its infrastructure backbone and federation to incorporate additional simulators. However, CARMA primarily focuses on simulating realistic V2X data.

Besides CARMA, other multi-resolution simulators like OpenCDA and OpenCDA-ROS exist, which simulate cooperative driving automation with background vehicles controlled by SUMO. They refine the original co-simulation platforms for CARLA and SUMO, with enhancements to simulate and assess online perception and planning under cooperative driving automation more accurately. Some platforms prioritize simulating communication delay with background vehicle control. One such instance, developed as a co-simulation platform between Webot, SUMO, and OMNet++, facilitates ego vehicle control via Webot while evaluating communication delays simulated by OMNet++ based on 802.11p. It's crucial to note that none of the multi-resolution simulation platforms incorporate specialized vehicle simulators like IVRESS and CarSim. This implies that vehicle-level simulation in these platforms is solely reliant on one-stop simulators like CARLA or Webot. For researchers requiring higher resolution beyond vehicle-level simulation, the capabilities of the aforementioned one-stop simulators may be inadequate.

In short, co-simulation shows advantages in simulating autonomous vehicles, as a single simulator lacks the capability to cover all aspects, and microscopic traffic simulators lacks certain level of fidelity with regard to vehicle level data. However, these co-simulation platforms still have limitations. Many simulators, while capable of co-simulating with some, cannot co-simulate with others due to various constraints like operating systems, computing platforms, or software compatibility issues. Therefore, BlueICE addresses these challenges by introducing a novel architecture for multi-modality simulation, detailed in the subsequent sections of this paper.

The BlueICE architecture is inspired by the Scalable Open Architecture for Embedded Edge (SOAFEE)\cite{RefWorks:RefID:5-spencer2021soafee} from ARM to be easily modified and scalable. This section will break down the BlueICE architecture and explain how we decouple the dependencies between simulators, autonomous driving stacks, operating systems, and the computing platform.


Figure \ref{fig:BigOverview} demonstrates BlueICE's architectural overview. BlueICE is divided into:
\begin{itemize}
    \item The Computing Layer.
    \item The Abstraction and Containerization Layer.
    \item The Communications Layer.
    \item The Applications Layer.
\end{itemize}
Each layer is pivotal in how BlueICE can be integrative and customizable. The Computing Layer decouples the dependencies between software and hardware using a cloud-native approach; the Abstraction and Containerization Layer, Communications Layer, and Applications Layer enable easy customization. Next, we will break down each layer and explain it in detail. 

\subsubsection{The Computing Layer}

The Computer Layer contains a heterogeneous computing platform, shown in \textbf{Fig \ref{fig:compute}}. BlueICE accomplishes this by creating the platform in the cloud. This gives us easier control over the drivers and the hardware. Because different autonomous driving stacks, testbeds, benchmarks, and simulators run on different computing platforms, BlueICE utilizes the heterogeneous platform to accomplish the following goals:

\begin{itemize} 
    \item  Performance and Efficiency: Different processing units are optimized for specific workloads. For example, GPUs excel at parallel processing, making them well-suited for graphics rendering and deep learning algorithms. CPUs, on the other hand, are better for general-purpose computation. By using the right processing unit for each task, a heterogeneous platform can achieve higher performance and energy efficiency than relying solely on a single processor type.

    \item Parallelism: Heterogeneous platforms can simultaneously take advantage of task-level parallelism, data-level parallelism, and instruction-level parallelism. This allows multiple tasks to be executed in parallel, leading to faster overall processing and reduced execution time.

    \item Flexibility: Different applications have varying computational requirements. A heterogeneous platform can adapt to different workloads by dynamically allocating tasks to the most suitable processing units. This flexibility enables the platform to handle a wide range of applications efficiently.

    \item Specialized Acceleration: Heterogeneous platforms can incorporate specialized hardware accelerators, such as FPGAs or ASICs, for specific functions like cryptography, signal processing, or machine learning. These accelerators can significantly boost the performance of specific workloads.

    \item Power Efficiency: The platform can achieve better power efficiency since each processing unit is optimized for specific tasks. For example, a GPU might perform tasks with much lower power consumption than a CPU.

    \item Future-Proofing: The computing landscape constantly evolves, with new algorithms, technologies, and computing paradigms emerging. Heterogeneous platforms offer a degree of future-proofing as they can adapt to new technologies by incorporating specialized hardware.

    \item Cost-Effectiveness: Heterogeneous platforms can offer cost savings by allowing designers to choose the most cost-effective processing units for specific tasks. Using specialized accelerators for computationally intensive workloads is often more cost-efficient than relying on a more expensive general-purpose processor.
\end{itemize}

\subsubsection{Abstraction and Containerization Layer}


The second layer is the Abstraction and Containerization Layer, shown in \textbf{Fig \ref{fig:contain}}. This layer is the main customization layer. Depending on the desired applications, BlueICE creates different containerized environments. Different containers will include different drivers and software versions. Making changes in one container does not affect other containers, and one can easily migrate or copy the container to another supported machine. This helps with isolation and deployment. Through abstraction and containerization, BlueICE achieves the following goals:

\begin{itemize}
    \item Portability: Containers encapsulate applications and their dependencies, making them portable across different environments. Developers can build once and run anywhere, reducing compatibility issues and easing the deployment process.

\item Isolation: Each component runs within its own container, ensuring isolation from other components and the underlying system. This enhances security, stability, and fault tolerance.

\item Scalability: Containers allow easy scaling by replicating instances of components as needed. With container orchestration platforms like Kubernetes, automatic scaling based on demand is feasible, improving resource utilization.

\item Resource Efficiency: Containers share the host OS kernel, leading to less resource overhead than traditional virtual machines. This results in efficient use of hardware resources and lower operational costs.

\item Faster Deployment: Containers are lightweight and start quickly, enabling rapid deployment and continuous integration/continuous deployment (CI/CD) pipelines. Developers can iterate faster and release updates more frequently.

\item Version Control and Rollback: Containers enable versioning, making it easier to control and roll back to specific versions when necessary. This enhances the reliability of the system and simplifies troubleshooting.

\item Dependency Management: Containers package all dependencies, ensuring consistency across various environments. Developers can avoid "works on my machine" issues, leading to a more reliable development process.

\item Easy Testing and Debugging: Containers provide a consistent and reproducible environment, simplifying testing and debugging efforts. Developers can test in environments that closely resemble the production setup.

\item Microservices Architecture: Containerization aligns well with microservices architecture, where each component can be containerized independently, enabling better maintainability and scalability of the entire system.

\item Ecosystem Support: Containerization has a robust ecosystem, with container registries, continuous integration tools, monitoring solutions, and cloud platforms all supporting containerized applications, simplifying development and operations.

\end{itemize}

\subsection{Communications Layer}
\subsubsection{Communication protocols used in BlueICE}

The third layer is the communications layer. In BlueICE, we use ROS as the communication protocol. Users can choose to use ROS1, ROS2, or both, depending on the services added to the final layer. ROS connects independent containers and applications with subscriptions and publication services. BlueICE synchronizes and orchestrates the information needed by and output given to different applications. One of its key advantages is its modular and distributed architecture, enabling seamless integration. A simplified view is shown in \textbf{Fig \ref{fig:rosbus}}. Application A, B, and C publish information onto the ROS bus for other simulators to use; they also subscribe to information on the ROS bus to use.

\subsubsection{Information Synchronization}

Data synchronization between containers and applications is crucial in testing and validation; it is especially important in BlueICE because it integrates so many containers. To resolve the issue with data synchronization, BlueICE uses the ROS clock from the communications layer, and all containers share the ROS clock. The simulated world will tick forward only and only if it has received a response from all of the integrated simulators. A simplified view is shown in \textbf{Fig \ref{fig:rosnodelay}}. 

Here, we see each simulator sharing a Master Clock. Application A takes some input from Application B and supplies some output for Application C. The process is the same for Application B and C. However, as previously shown, in \textbf{Fig \ref{fig:rosbus}}, this is not a direct communication, and everything is published onto the same ROS bus. This simplifies the process of adding a new application - create a subscription service to the information needed.

\subsubsection{Communication delay simulation}

For data that includes delays, such as network packages, the synchronization module pushes the message back until it has waited for the calculated delay so that it will not block the other simulators. A simplified view is shown in \textbf{Fig \ref{fig:rosyesdelay}}, where it shows Application C waits, for the duration of the delay, to send the message; but Application C does not stop the other parts as it is still synchronized to the Master Shared Clock.


\subsection{Application Layer}

Last, the application layer is where users connect BlueICE with their applications. The applications communicate via the ROS bus, as shown in \textbf{Fig \ref{fig:rosbus}}. The underlying architecture supports a plethora of applications all of which can be integrated into BlueICE via the same integration mechanisms mentioned above. 

Autoware.Universe\cite{RefWorks:RefID:13-kato2018autoware} is the standard autonomous driving stack to use, and users can freely replace any of the components to suit their research needs.  

This section features the preliminary designs and findings of our Digital Twin at the University of Delaware D-STAR campus. D-STAR is a campus-scale mobility testbed at UD STAR Campus, which includes a Cisco private 5G network, C-V2X infrastructure from iSmartways and Danlaw Inc., and DELL edge servers. Specifically, D-STAR has five C-V2X Roadside Units (RSU), which will be deployed on the campus, serving more than 23,000 residents and covering four large parking structures and more than 20 parking lots. The D-STAR testbed can support the communication and collaboration between vehicles, edge devices, and the cloud. The overarching goal of the D-STAR testbed is fueling the campus-wide collaboration on connected and sustainable mobility research and education.

\subsection{Digital Twin at the University of Delaware (D-STAR)}

Combined with real-world data, BlueICE can be used to create a digital twin for autonomous driving testing. \textbf{Fig \ref{fig:digitaltwinoverview}} demonstrates the high-level overview of the digital twin we are building at the University of Delaware STAR campus. 

In this digital twin testing environment, we are mainly concerned with the environment, the test vehicle, the background road users, and the cellular network. 

D-STAR leverages BlueICE's heterogenous computing platform layer and abstraction layer to containerize and combine the GPU-intensive simulator, the CPU-intensive network simulator and traffic simulator,  HPC-based machines for weather and ground simulation, and x86-architecture and ARM64-architecture machines together.

BlueICE also orchestrates the input, output, and data synchronization between the different containers, shown in \textbf{Fig \ref{fig:trans}}. All of the individual boxes represent a part of the digital twin that can be containerized and replaced. For example, if a new camera synthetic data generation model is proposed, we can quickly replace and deploy the model in our digital twin.

CARLA is in a container on a GPU-intensive machine, NS-3, SUMO, and others are deployed in containers on a CPU-intensive machine, IVRESS and DDT are deployed in containers on a cloud HPC, and Autoware.Universe is deployed in containers both in the x86 and the ARM64 environment. \textbf{It is important to note that without the BlueICE architecture, this setup would be impossible to create.}

BlueICE manages the transactions between D-STAR and the real world by using the following:

\begin{itemize}
    \item An initial set of road and building meshes are created using OpenStreetMap, Roadrunner, and Google Satelite images. The roads and buildings are automatically updated when the test vehicle collects data.
    \item An initial weather is set in CARLA and is updated when cameras capture a change in the weather.
    \item An initial set of vehicle parameters, such as length, width, height, axis, and max steering angle is used to create a vehicle blueprint using Unreal Engine. CARLA's default physics model is updated as the test vehicle collects data when driving in the real world.
    \item A set of sensor parameters is given to CARLA to recreate the camera, LiDAR, GPS, and IMU sensors. The sensor parameters are based on the datasheet provided by the sensors' manufacturers. 
    \item Background road user movements, including vehicles and pedestrians, are captured using cameras and LiDARs and replayed using SUMO.
    \item Traffic information is modeled and controlled by SUMO. SUMO can either replay recorded data from the infrastructure's cameras or generate unknown traffic scenarios.
    \item Network information for 5G and C-V2X, such as latency and packet loss rate, are initially modeled using NS-3. Multiple sets of Road-Side-Units (RSU) and OnBoard-Units (OBUs) relay the network information to update network models.
    \item The autonomous driving stack, Autoware.Universe, uses the same vehicle and sensor parameters to generate vehicle commands. We set up a Vehicle-in-the-Loop test by supplying the vehicle sensors with simulated inputs and using the actual vehicle to output control commands to control the sim-vehicle in simulation.
\end{itemize}

\subsubsection{The Environment}


The road network is recreated by taking the OpenStreetMap (OSM) file and feeding it into OpenDrive (XODR) to create the roads, the sidewalks, the intersections, and the infrastructure. We created a pipeline, shown in \textbf{Fig \ref{fig:updateroad}}, that updates the road conditions with LiDAR and camera information. We take the default road built by OpenDrive and CARLA, update the friction model with recorded data, and use the recorded LiDAR and camera data to update the potholes and pools of water on the road to automatically update the road conditions. This ensures that when the simulated autonomous vehicle is under test, the simulated road conditions represent that of the real world.


For the buildings, we created a pipeline that takes images and videos as inputs and outputs the 3D meshes of the buildings. \textbf{Fig \ref{fig:buildsandmap}} shows a few examples of the generated buildings from our pipeline, as shown in \textbf{Fig \ref{fig:updatebuildings}}.

This pipeline is more than creating the meshes for the buildings, it is also responsible for \textbf{updating the digital twin map}. In our research, we could not find any tools or publications that touched upon automatically updating simulated environments. The lack of this automated process resulted in huge amounts of manual effort or digital twins becoming outdated and obsolete when constructions change the environment. Our pipeline tackles this by taking the recorded images and videos from our test vehicle or aerial drones, creates new meshes for the buildings, verifies that it is different from the existing map, and updates the existing map. We also manually verify that the meshes created represent the actual buildings. This ensures that our map is always up-to-date and reflects the real world.


The weather is also another very important aspect of the environment. The initial implementation is done using CARLA's weather engine. Some example weather conditions are shown in \textbf{Fig \ref{fig:weather}}. We also built a pipeline that uses camera data and a pre-trained weather model to update the weather conditions in CARLA. This gives us close-to-reality camera sensor readings in different weather conditions.

\subsubsection{The Vehicle}

The vehicle under test(VUT) is our Hydra platform, as shown in \textbf{Fig \ref{fig:thecar}}. Multiple parts of the vehicle need to be simulated in the digital twin: the LiDAR, GPS/IMU, and camera sensors, the vehicle dynamics, the drive-by-wire (DBW) controls, and the autonomous driving algorithms. The combination of the vehicle parameters and sensor parameters allows D-STAR to simulate the vehicle as close to the test vehicle as possible.

The camera sensor parameters are shown in \textbf{Table \ref{tab:camera}}, the lidar sensor parameters in \textbf{Table \ref{tab:lidar}}, the GPS sensor in \textbf{Table \ref{tab:gps}}, the IMU sensor in \textbf{Table \ref{tab:imu}}, and the DBW and vehicle dynamics in \textbf{Table \ref{tab:dbw}}.

% 

\subsubsection{Background Road Users}

As previously introduced in section \ref{LR:micro_sim} and \ref{LR:vehicle_sim}, both microscopic level simulators and vehicle level simulators can generate and control background road users. For synchronization of vehicle motion between vehicle simulator and microscopic traffic simulators, usually the background vehicle is fully controllable by only one simulator, and for other simulator it creates a digital replicate of the background vehicle and the motion of such background vehicle is replicated according to the newest simulation result. This mechanism include coordinate synchronization and time synchronization, and the synchronization between microscopic traffic simulator and vehicle simulator ensure the performance consistency for both VUT and background vehicles.

The background traffic represents a group of traffic participants which shared similar patterns to some extend. For example, they can governed by the same car-following model when driving on freeway, or they can perform similar lane-change maneuvers which shares the same underlying lane change decision and trajectory planning model. 


In such context, it is possible to simulate a mixed traffic pattern with different underlying models governed by microscopic traffic simulators. From microscopic traffic simulators, users can pre-define various traffic models with different parameters to create a mixed traffic pattern. For example, different levels of reaction times can be defined for car-following models, different levels of eagerness in lane change can be defined for lane-change models, different levels of aggressive can be defined through time-headway for both car-following models and junction models in SUMO \cite{SUMOsafety}. This leads to a higher variation in background traffic and bridge the gap between the performance of VUT in simulation to the performance of VUT in real-world, as background traffic is less predictable in real-world comparing background traffic governed by same control and motion model.

Also, it should be noted that not all background road users can send C-V2X message to the VUT. This is also a setting that is close to the real-life scenarios, as not all vehicles are equipped with CV2X communication devices. In such sense, although all background road users are controllable by the microscopic traffic simulator(in our case, we chose SUMO), not all background vehicles can share their state and intention with VUT. This can be regulated on SUMO side by selectively publish vehicle state information onto the communication layer, where only certain kinds of road users messages will be shared. Also, the communication delay between background road users and VUT can also be simulated and replicated by BlueICE. Such mechanism will be discussed in detail in the next paragraphs.




\subsubsection{Network and Communication}

Vehicle-to-Everything (V2X) technologies show great potential to increase the safety of autonomous vehicles, D-STAR chose 6 intersections to install new C-V2X-enabled infrastructure. Multiple OBUs are placed around the campus to collect latency and packet loss information. 

In order for the vehicles and infrastructure to communicate inside the simulation, all C-V2X messages are converted from ASN.1 format to ROS2 messages. All of the standard J2735 messages are recreated using ROS2. When any unit broadcast or receive a message, D-STAR uses the OBU closest to the unit, in terms of world coordinate, to report the latency and packet loss rate. That latency is then used to delay the package received time. The delay simulated by BlueICE is based on the actual experimental data collected in UDel.

\subsubsection{Workflow}


The workflow and information flow are shown in Fig \ref{fig:simworkflow}. Before the simulation starts, environment information is given to the sim-environment to update the roads, buildings, and weather; vehicle dynamics and point cloud (PCD) map are given to the sim-vehicle and Autoware. 

When the simulation begins, the sim-vehicle generates the GPS and IMU sensor data and the sim-environment generates the LiDAR and camera data; these data are given to Autoware to perform localization, object detection, path planning, and other autonomous driving applications. Autoware outputs the vehicle control commands to control the sim-vehicle. The new sim-vehicle position will result in the sim-vehicle and the sim-environment generating different data. Autoware also broadcasts some C-V2X messages to the surrounding infrastructure. In the real world environment, based on the sim-vehicle location, find the closest OBU and use the reported latency to determine the C-V2X message delay. The infrastructure also broadcasts C-V2X messages, based on the sim-vehicle location, finds the closest OBU, and uses the reported latency to determine the C-V2X message delay. Then, the sim-vehicle receives the delayed message and uses the contents for its applications.


\subsubsection{Evaluation and Results}

First, pipeline-built building meshes are evaluated. Previously, building meshes in digital twins were built by 3D artists. This is the first time researchers have used generated meshes. Therefore, we first need to verify that, visually, the generated meshes is similar to the actual building.


In \textbf{Fig \ref{fig:meshcomp}}, an image of the UD Modular lab is shown on the top, 3D meshes built by Google Earth are shown on the bottom left, and 3D meshes built by our pipeline are shown on the bottom right. We can see that structurally, most of the building is reconstructed correctly in the generated mesh. There are a few partial-missing representations, such as the ramp in front of the main entrance, but when compared to Google Earth, which also used a series of images to reconstruct the meshes, is very similar.

Simply doing a visual examination is not enough. We need to go beyond "it looks real" to "it behaves real". Therefore, we also need to verify that the reconstructed 3D meshes reflect the correct LiDAR point clouds.


In \textbf{Fig \ref{fig:lidarcomp}}, the point cloud map shown in white in both images is built from real LiDAR data points collected by our test vehicle with the VLP-16 LiDAR. The left image demonstrates the vehicle localizing using real data, and the right image demonstrates the simulated vehicle using simulated LiDAR data to localize. The difference between the ground truth position and the localized position in simulation is smaller than 5 cm. These results prove our reconstructed 3D meshes "look real" and "behave real". We can confidently conclude that our pipeline to perform automatic mesh updates and D-STAR building meshes are usable and accurate.


Next, we move on to Traffic simulation. To test our autonomous driving algorithms without being a safety threat to the surrounding community, we can utilize this road segment as a proving ground, and create virtual background traffic using the concept of augmented reality shown in \cite{8500545}. \textbf{Fig \ref{fig:sumogen}} shows the SUMO interface creating and controlling traffic using background vehicle models. \textbf{Fig \ref{fig:gentraffic}} takes a snapshot of the scene after SUMO has generated some background road users. Then in \textbf{Fig \ref{fig:autowaresnap}}, we demonstrate a snapshot of our integrated autonomous driving stack, Autoware.Universe.


\subsubsection{Future Work and other potential applications}

We did not have the chance to thoroughly test our pipeline to update potholes on roads but our preliminary implementation using the BlueICE architecture has already made D-STAR a state-of-the-art digital twin; it is the first digital twin to use a pipeline to automatically generate and update buildings' 3D meshes.

But D-STAR is far from a perfect representation. As we continue to integrate more and more simulators in containers, it will be as close to perfect as possible. With the extreme amount of data generated by different simulators, D-STAR will trade its speed for accuracy, becoming the most precise digital twin for autonomous driving testing.


Before D-STAR gets there, there are a few other potential applications for D-STAR. \textbf{Fig \ref{fig:medriving}} demonstrates our human-in-the-loop autonomous driving platform. Other applications such as pedestrian detection, smart cities, and smart transportation show great potential on D-STAR.

We are also working on creating the UDrive benchmark for connected and autonomous vehicles. The benchmark systematically classifies and generates test cases ranging from common to edge case driving scenarios.


% \textcolor{red}{change}
%%%Improvement on architecture(BlueICE) itself
We have demonstrated the UD-DT to show that the BlueICE architecture can be used to create a highly accurate digital twin. In this section, we will briefly discuss some of the disadvantages and our future work.

Being integrative and customizable comes with a heavy price tag - latency. Containerizing the different components will certainly increase the processing time by a great deal, and the latency will only increase if BlueICE integrates more specialized simulators. Even though researchers generally do not concern themselves with latency in testing and validation, one might need to integrate a driving simulator that requires real-time data generation. BlueICE, being cloud-native, can be sped up by adding more processing power.

One of our future works involves continuing to integrate more specialized simulators. Many specialized simulators do not use ROS, therefore, we will work towards making a ROS bridge for all of the popular open-source simulators.

We will also continue to improve the usability of BlueICE by adding new GUI interfaces to help users decide what combination of simulators is best for their research needs.

For our digital twin at the University of Delaware STAR campus, we plan to also improve and design new benchmarks for future autonomous driving systems, where they will be scored based on safety and passenger comfort levels.

This paper introduced the BlueICE architecture, an integrative and customizable architecture to support high-fidelity realistic autonomous driving testing. BlueICE accomplishes this goal by decoupling the dependencies between simulators, platforms, and autonomous driving stacks. BlueICE allows seamless co-simulation between previously incompatible simulators through the cloud-native heterogeneous platform layer and the abstraction layer; BlueICE also manages and orchestrates the data flow and synchronization using the ROS2 protocols.

This paper also demonstrated the University of Delaware digital twin. We thoroughly discussed the different components of BlueICE and how they play into making the UD-DT a state-of-the-art digital twin for autonomous vehicle testing. The results from the UD-DT have shown that it is precise and can be used to evaluate autonomous vehicles.

We are convinced that as we continue to perfect the BlueICE architecture and integrate more simulators into the UD-DT, every autonomous vehicle researcher and interested member will be able to confidently test, validate, and deploy their applications without owning an autonomous vehicle.
